Choose Your Lenses: Flaws in Gender Bias Evaluation

Considerable efforts to measure and mitigate gender bias in recent years have led to the introduction of an abundance of tasks, datasets, and metrics used in this vein. In this position paper, we assess the current paradigm of gender bias evaluation and identify several flaws in it. First, we highlight the importance of extrinsic bias metrics that measure how a model's performance on some task is affected by gender, as opposed to intrinsic evaluations of model representations, which are less strongly connected to specific harms to people interacting with systems. We find that only a few extrinsic metrics are measured in most studies, although more can be measured. Second, we find that datasets and metrics are often coupled, and discuss how their coupling hinders the ability to obtain reliable conclusions, and how one may decouple them. We then investigate how the choice of the dataset and its composition, as well as the choice of the metric, affect bias measurement, finding significant variations across each of them. Finally, we propose several guidelines for more reliable gender bias evaluation.

==> bios-table.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lllll}
\toprule
                & \multicolumn{4}{c}{\textbf{Debiasing Strategy}} \\
\cmidrule{2-5}
\textbf{Metric} & None & Oversampling & Subsampling & Scrubbing \\
\midrule
Compression & 4.121 $\pm$ 1.238 & 8.522* $\pm$ 2.354 & 3.568 $\pm$ 1.516 & \textbf{1.699}* $\pm$ 0.138\\
Accuracy &  \textbf{0.861} $\pm$ 0.005 & 0.852* $\pm$ 0.004 & \textbf{0.861} $\pm$ 0.003 & 0.851* $\pm$ 0.003 \\
TPR gap (P) &  0.763 $\pm$ 0.071 & 0.729 $\pm$ 0.067 & \textbf{0.319}* $\pm$ 0.114 & 0.704* $\pm$ 0.068 \\
TPR gap (S) &  2.391 $\pm$ 0.257 & 2.145* $\pm$ 0.220 & \textbf{1.598}* $\pm$ 0.273 & 2.019* $\pm$ 0.262 \\
FPR gap (P) &  0.591 $\pm$ 0.052 & 0.491* $\pm$ 0.059 & \textbf{0.087}* $\pm$ 0.094 & 0.552 $\pm$ 0.063 \\
FPR gap (S) &  0.075 $\pm$ 0.010 & 0.085* $\pm$ 0.011 & \textbf{0.030}* $\pm$ 0.006 & 0.057* $\pm$ 0.007 \\
Precision gap (P) &  0.398 $\pm$ 0.053 & 0.327* $\pm$ 0.044 & \textbf{0.166}* $\pm$ 0.055 & 0.347* $\pm$ 0.050 \\
Precision gap (S) &   0.015 $\pm$ 0.001 & 0.015 $\pm$ 0.001 & \textbf{0.011}* $\pm$ 0.001 & 0.013* $\pm$ 0.001 \\
Independence gap (S) &  0.009 $\pm$ 0.002 & 0.008 $\pm$ 0.002 & \textbf{0.001}* $\pm$ 0.000 & 0.005* $\pm$ 0.001 \\
Separation gap (S) &  0.327 $\pm$ 0.051 & 0.305 $\pm$ 0.030 & \textbf{0.204}* $\pm$ 0.032 & 0.296 $\pm$ 0.053 \\
Sufficiency gap (S) &  9.451 $\pm$ 1.945 & 8.324* $\pm$ 1.537 & \textbf{1.218}* $\pm$ 0.330 & 4.930* $\pm$ 0.927  \\
\bottomrule
\end{tabular}
    \caption{Occupation Prediction: Results on a RoBERTa-based model trained over 10 seeds. Significant reduction or increase in a metric ($p < 0.05$ on Pitman's permutation test), compared to the non-debiased model (debiasing strategy is None), is marked with *. The lowest bias score or highest performance metric in each column is marked with \textbf{bold}. P = Pearson; S = Sum.}
    
    \label{bios-finetuning}
\end{table*}

==> coref-table.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{lllll}
\toprule
                & \multicolumn{4}{c}{\textbf{Debiasing Strategy}} \\
\cmidrule{2-5}
\textbf{Metric} & None & Anon & CA & Anon + CA \\
\midrule
F1 diff ($pro - anti$) & 6.631 $\pm$ 1.013 &  7.256 $\pm$ 0.846 & \textbf{2.302}* $\pm$ 0.466 &  2.422* $\pm$ 0.714 \\
TPR gap (P) &  0.654 $\pm$ 0.069 & 0.710* $\pm$ 0.047 & \textbf{0.607} 0.082 $\pm$ & 0.627 $\pm$ 0.100 \\
TPR gap (S) & 4.884 $\pm$ 0.698 & 4.870 $\pm$ 0.509 & 2.041* $\pm$ 0.228 & \textbf{2.014}* $\pm$ 0.286 \\
FPR gap (P) & 0.602 $\pm$ 0.036 & 0.620 $\pm$ 0.056 & \textbf{0.572} $\pm$ 0.078 & 0.629 $\pm$ 0.107 \\
FPR gap (S) &  0.120 $\pm$ 0.015 & 0.128 $\pm$ 0.011 & 0.050* $\pm$ 0.006 & \textbf{0.049}* $\pm$ 0.007 \\
Precision gap (P) & 0.654 $\pm$ 0.068 & 0.710* $\pm$ 0.048& \textbf{0.607} $\pm$	0.083 & 0.627 $\pm$	0.099 \\
Precision gap (S) & 0.061 $\pm$ 0.009 & 0.061 $\pm$ 0.006 & 0.026* $\pm$ 0.003 & \textbf{0.025}* $\pm$ 0.004 \\
Independence gap (S) &  0.027 $\pm$ 0.008 & 0.025 $\pm$ 0.004 & \textbf{0.004}* $\pm$ 0.001 & \textbf{0.004}* $\pm$ 0.001\\
Separation gap (S) & 1.247 $\pm$ 0.150 & 1.344 $\pm$ 0.137 & \textbf{0.537}* $\pm$ 0.061	& 0.557* $\pm$ 0.070\\
Sufficiency gap (S) &  8.684 $\pm$ 1.883 & 8.816 $\pm$ 1.544 & 1.673* $\pm$ 0.354	& \textbf{1.557}* $\pm$ 0.384 \\
\bottomrule
\end{tabular}
    \caption{Coreference resolution: results on Ontonotes test set and Winobias challenge set. Each model was trained over 10 seeds. * Marks significant reduction or increase in bias ($p < 0.05$ on Pitman's permutation test), compared to the non-debiased model (debiasing strategy None). The lowest bias score or highest performance metric in each column is in \textbf{bold}. P = Pearson; S = Sum.}

    \label{coref-finetuning}
\end{table*}


==> extrinsic_metrics_count_table.tex <==
\begin{table}

\centering

\begin{tabular}{cc}
\toprule
\multicolumn{1}{l}{Maximum \# of extrinsic} & \# of papers \\
\multicolumn{1}{l}{metrics per task} &  \\
\midrule
0 & 13 \\
1 & 8 \\
2 & 7 \\
3 & 6 \\
6 & 1 \\
10 & 1 \\
\bottomrule
\end{tabular}

\caption{Papers about gender bias and the number of extrinsic metrics they measured per task. 0 means no extrinsic metrics were measured.}
\label{tbl:extrinsic_count}
\end{table}
